New Trends for Modern Machine Translation with Large Reasoning Models

Recent advances in Large Reasoning Models (LRMs), particularly those leveraging Chain-of-Thought reasoning (CoT), have opened brand new possibility for Machine Translation (MT). This position paper argues that LRMs substantially transformed traditional neural MT as well as LLMs-based MT paradigms by reframing translation as a dynamic reasoning task that requires contextual, cultural, and linguistic understanding and reasoning. We identify three foundational shifts: 1) contextual coherence, where LRMs resolve ambiguities and preserve discourse structure through explicit reasoning over cross-sentence and complex context or even lack of context; 2) cultural intentionality, enabling models to adapt outputs by inferring speaker intent, audience expectations, and socio-linguistic norms; 3) self-reflection, LRMs can perform self-reflection during the inference time to correct the potential errors in translation especially extremely noisy cases, showing better robustness compared to simply mapping X->Y translation. We explore various scenarios in translation including stylized translation, document-level translation and multimodal translation by showcasing empirical examples that demonstrate the superiority of LRMs in translation. We also identify several interesting phenomenons for LRMs for MT including auto-pivot translation as well as the critical challenges such as over-localisation in translation and inference efficiency. In conclusion, we think that LRMs redefine translation systems not merely as text converters but as multilingual cognitive agents capable of reasoning about meaning beyond the text. This paradigm shift reminds us to think of problems in translation beyond traditional translation scenarios in a much broader context with LRMs - what we can achieve on top of it.

==> signlanguage.tex <==
QvQ-72B-preview

Answer

So I'm trying to figure out what number this hand sign represents in American Sign Language (ASL). Let me see... In ASL, each number from 0 to 10 has its own unique hand shape, and it's important to recognize them correctly.

First, I need to observe the hand position. The thumb is bent and touching the base of the index finger, and then the index, middle, and ring fingers are extended straight up. The pinky is also extended, but it seems like it might be slightly bent or not as straight as the other fingers. The palm is facing towards me.

Let me recall the ASL numbers. Starting from zero:

0: Fist, thumb touches the pinky.
1: Index finger extended, rest are closed.
2: Index and middle fingers extended.
3: Index, middle, and ring fingers extended.
4: Index, middle, ring, and pinky extended.
5: All fingers extended.
6: All fingers extended, thumb touches the side of the index finger.
7: All fingers extended, thumb crosses over to touch the middle finger.
8: All fingers extended, thumb touches the ring finger.
9: All fingers extended, thumb touches the pinky.
10: Both hands showing 5.
Looking at this, the hand has the thumb bent and touching near the index finger, and four fingers extended: index, middle, ring, and pinky. Wait, but in the description, it says the pinky is slightly bent. Maybe it's not fully extended like the other fingers.

In ASL, the number 4 is shown with all four fingers extended and the thumb touching the base of the index finger. That seems similar to what's being shown here. But I need to make sure.

Let me check again: thumb is bent and touching near the index finger, and the index, middle, ring, and pinky are extended. If the pinky is slightly bent, maybe it's still considered as extended for the purpose of the sign.

Alternatively, maybe it's the number 9, which also involves the thumb touching the pinky while all fingers are extended. But in 9, the thumb touches the pinky, whereas in 4, the thumb touches the base of the index finger.

Wait, according to the standard ASL hand shapes, number 4 is indeed the hand with the thumb touching the base of the index finger and the four fingers extended.

Number 9, on the other hand, has all five fingers extended with the thumb touching the pinky.

So, in the image, if the thumb is touching near the index finger and four fingers are extended, it should be the number 4 sign in ASL.

But I'm a bit confused because I thought in number 9, the thumb touches the pinky while all fingers are extended. Maybe the description is a bit unclear about the exact position of the thumb.

Let me try to visualize this again. Thumb is bent and touching the base of the index finger, and the index, middle, ring, and pinky are extended. That matches the description of number 4 in ASL.

Number 9 would have all five fingers extended, with the thumb touching the pinky, which isn't the case here since the thumb is touching the base of the index finger.

Therefore, the hand sign in the image represents the number 4 in American Sign Language.

Final Answer

4
4
​

